MERLOT Reserve: Neural Script Knowledge through Vision and Language and Sound

As humans, we navigate a multimodal world, building a holistic understanding from all our senses. We introduce MERLOT Reserve, a model that represents videos jointly over time -- through a new training objective that learns from audio, subtitles, and video frames. Given a video, we replace snippets of text and audio with a MASK token; the model learns by choosing the correct masked-out snippet. Our objective learns faster than alternatives, and performs well at scale: we pretrain on 20 million YouTube videos. Empirical results show that MERLOT Reserve learns strong multimodal representations. When finetuned, it sets state-of-the-art on Visual Commonsense Reasoning (VCR), TVQA, and Kinetics-600; outperforming prior work by 5%, 7%, and 1.5% respectively. Ablations show that these tasks benefit from audio pretraining -- even VCR, a QA task centered around images (without sound). Moreover, our objective enables out-of-the-box prediction, revealing strong multimodal commonsense understanding. In a fully zero-shot setting, our model obtains competitive results on four video tasks, even outperforming supervised approaches on the recently proposed Situated Reasoning (STAR) benchmark. We analyze why audio enables better vision-language representations, suggesting significant opportunities for future research. We conclude by discussing ethical and societal implications of multimodal pretraining.

==> figures/imagenet_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht!]
\centering
\caption{Zero-shot accuracy on ImageNet-1K with ViT-B/32.}
\begin{tabular}{@{}lcc@{}}

Model   & Top-1 Acc (\%) & Top-5 Acc (\%) \\ \toprule
\modelname & 7.29          & 20.33         \\
CLIP     & 58.88         & 85.61         \\ \bottomrule
\end{tabular}
\label{tab:imagenettable}
\end{table}

==> figures/star_table.tex <==
\begin{table}[t]
\begin{tabular}{@{\hspace{0.05cm}} p{3.0 cm} @{\hspace{0.05cm}} p{0.95cm} @{\hspace{0.05cm}} p{0.95cm} @{\hspace{0.05cm}} p{0.95cm} @{\hspace{0.01cm}} p{0.95cm} @{}}
&  \multicolumn{4}{c}{\hspace{15mm}{\scriptsize STAR (acc; \%) }} \\
Model & Inter & Seq & Pred & Fea \\ \toprule
% & CNN-LSTM       & 33.25       &   32.67 & 30.69 & 30.43 \\
% & CNN-BERT      & 33.59 &  37.16  & 30.95 &  30.84\\ 
% \midrule
NS-SR \cite{wu2021star} & 30.9 & 31.8 & 30.2 & 29.7 \\
L-GCN \cite{hu2019language} & 39.0 & 38.0 & 28.8 &  27.0\\
HCRN \cite{le2020hierarchical} & 39.1 & 38.2 & 28.8 & 27.3 \\
ClipBERT \cite{lei2021less} & 39.8 &  \textbf{43.6} & 32.3 &  31.4 \\
\midrule
\basemodel$^\texttt{w/o audio}$ & 44.4 & 40.1 & 38.1 & 35.0 \\
\largemodel$^\texttt{w/o audio}$ &  42.6 & 41.1 &  37.4 & 32.2 \\
\basemodel & \textbf{44.8} & 42.4 & \textbf{38.8} & \textbf{36.2}\\
\largemodel & 43.9 & 42.6 & 37.6 & 33.6 \\
\bottomrule
\end{tabular}\vspace{-1mm}
\caption{\modelname gets state-of-the-art results on STAR with \textbf{zero-shot} by a margin of \textbf{over 3.7\%}, over methods from prior \textbf{supervised} method.}
\label{tab:startablefull}
\end{table}

